Detecting and Counting Small Subgraphs, and Evaluating a Parameterized Tutte Polynomial: Lower Bounds via Toroidal Grids and Cayley Graph Expanders

Given a graph property $\Phi$, we consider the problem $\mathtt{EdgeSub}(\Phi)$, where the input is a pair of a graph $G$ and a positive integer $k$, and the task is to decide whether $G$ contains a $k$-edge subgraph that satisfies $\Phi$. Specifically, we study the parameterized complexity of $\mathtt{EdgeSub}(\Phi)$ and of its counting problem $\#\mathtt{EdgeSub}(\Phi)$ with respect to both approximate and exact counting. We obtain a complete picture for minor-closed properties $\Phi$: the decision problem $\mathtt{EdgeSub}(\Phi)$ always admits an FPT algorithm and the counting problem $\#\mathtt{EdgeSub}(\Phi)$ always admits an FPTRAS. For exact counting, we present an exhaustive and explicit criterion on the property $\Phi$ which, if satisfied, yields fixed-parameter tractability and otherwise $\#\mathsf{W[1]}$-hardness. Additionally, most of our hardness results come with an almost tight conditional lower bound under the so-called Exponential Time Hypothesis, ruling out algorithms for $\#\mathtt{EdgeSub}(\Phi)$ that run in time $f(k)\cdot|G|^{o(k/\log k)}$ for any computable function $f$. As a main technical result, we gain a complete understanding of the coefficients of toroidal grids and selected Cayley graph expanders in the homomorphism basis of $\#\mathtt{EdgeSub}(\Phi)$. This allows us to establish hardness of exact counting using the Complexity Monotonicity framework due to Curticapean, Dell and Marx (STOC'17). Our methods can also be applied to a parameterized variant of the Tutte Polynomial $T^k_G$ of a graph $G$, to which many known combinatorial interpretations of values of the (classical) Tutte Polynomial can be extended. As an example, $T^k_G(2,1)$ corresponds to the number of $k$-forests in the graph $G$. Our techniques allow us to completely understand the parametrized complexity of computing the evaluation of $T^k_G$ at every pair of rational coordinates $(x,y)$.

==> tikzlibraryconference.code.tex <==
%\documentclass{standalone}
%\usepackage{tikz}

\usepackage{ifthen}
\usetikzlibrary{calc,shapes,fit}
\usetikzlibrary{decorations.markings}


\tikzset{vertex/.style={circle, fill, inner sep=1pt, outer sep=1.3pt}}
\tikzset{svertex/.style={circle,draw=white, line width=1.2pt,fill=black, inner sep=1.8pt, outer sep=0pt}}
\tikzset{ssvertex/.style={circle,fill=black, inner sep=.7pt, outer sep=-.75pt}}
\tikzset{sssvertex/.style={circle,fill=black, inner sep=.5pt, outer sep=-.6pt}}
\tikzset{bbvertex/.style={circle,fill=black, inner sep=.8pt, outer sep=-.9pt}}
\tikzset{bag/.style={gray,minimum size=20pt,diamond,draw,rounded corners=4pt, inner sep=0pt, outer sep=-4pt, double=white, thick, fill=white}}
\tikzset{sbag/.style={gray,minimum size=15pt,diamond,draw,rounded corners=2pt, inner sep=0pt, outer sep=-4pt, double=white, thick, fill=white}}

%\tikzset{hom/.style={black}}
%\tikzset{shom/.style={white,double=black, thick}}

\def\ccol{red}
\def\ecol{blue}
\def\icol{red!50!blue}

\tikzset{ssedge/.style={white,thick, double=black, double distance=2pt}}
\tikzset{tedge/.style={white,thick, double=black, double distance=1pt}}
\tikzset{sssedge/.style={white,thick, double=black, double distance=1.5pt}}
\tikzset{stedge/.style={white,thin, double=gray, double distance=.6pt}}
\tikzset{sstedge/.style={white,thin, double=gray!60, double distance=.6pt}}
\tikzset{dedge/.style={gray,thick, double=white, double distance=9pt}}
\tikzset{sdedge/.style={gray,thick, double=white, double distance=5pt}}

\tikzset{sty/.store in=\sty,sty=10}

\tikzset{cross/.style={cross out, draw, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer         sep=0pt}}

\tikzset{tvertex/.style={circle, fill, inner sep=1pt, outer sep=1.3pt}}
\tikzset{btvertex/.style={draw,circle,dashed,very thin,gray,inner sep=4pt, outer sep=-1pt}}
\tikzset{bbtvertex/.style={draw,dashed,thin,gray,inner sep=5.5pt, outer sep=-.5pt}}

\def\dotedge[#1](#2)--(#3);{%
    \draw[#1,dotted] ($(#2)!.33!(#3)$) -- ($(#2)!.66!(#3)$);%
    \draw[#1] ($(#2)!.64!(#3)$) -- (#3);%
    \draw[#1] (#2) -- ($(#2)!.35!(#3)$);%
}

%% slice from pgfpie

% #8:#1 center
% #7:#2 radius
% #1:#3 begin angle
% #2:#4 end angle
% #5:#5 explode
% #6: fill color

% #3: number
% #4: label
% #6: fill color

\makeatletter
\tikzset{slsty/.store in=\@sty,slsty=}
\def\slice#1#2#3#4#5#6#7{
    \pgfmathsetmacro{\midangle}{0.5*(#3)+0.5*(#4)}
    \pgfmathsetmacro{\sliceradius}{#2+#5}
    \path (#1) -- ++(\midangle:#5) coordinate(O);
    \node[inner sep=1pt, outer sep=1.2pt] (#7) at (O) {};
    \draw[line join=round, color=#6, fill=#6, \@sty] (O) -- ++(#3:#2) arc (#3:#4:#2) -- cycle;
}

% #1 coordinate
% #2 split
% #3 coordinate name
\def\kowaen#1#2#3;{
    \foreach \i/\j/\k [count=\c from 1] in {#2} {
        \slice{#1}{1.3pt}{\i}{\j}{2pt}{\k}{#3-\c};
    }
}

\def\coledge(#1|#2)--(#3|#4);{
    \draw[tedge] (#1) -- (#3);
    \draw[tedge, double=#2] (#1) -- ($(#1)!.35!(#3)$);
    \draw[tedge, double=#4] (#3) -- ($(#3)!.35!(#1)$);
}

\tikzset{
    every label/.append style={font=\tiny, label distance=-3}
}

\tikzset{
    pics/torus/.style args={#1/#2}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\sty,10))}
            \pgfmathsetmacro{\mode}{int(\sty - \bg * 10)}

            \pgfmathsetmacro{\normalgrid}{#2==14}
            \ifthenelse{\mode=0}{
                % normal mode
                \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                \ifthenelse{\normalgrid=1}{
                    \def\vs{tvertex}
                    }{
                    \def\vs{btvertex}
                }
                \def\es{tedge}
                \def\ess{stedge}
                }{
                \ifthenelse{\mode=1}{
                    % grid where each vertex is split into 6 parts (for a 3d grid
                    \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                    \ifthenelse{\normalgrid=1}{
                        \def\vs{tvertex}
                        }{
                        \def\vs{bbtvertex}
                    }
                    \def\es{tedge}
                    \def\ess{stedge}
                    }{
                    % grid-colored graph (only supports 2d grids
                    \pgfmathsetmacro{\dist}{\bg==2?1.15:.9}
                    \def\vs{bag}
                    \def\es{dedge}
                    \def\ess{sdedge}
                }
            }
            \pgfmathsetmacro{\n}{int(#1-1)}

            \foreach\j in {1,...,#1} {
                \pgfmathsetmacro{\xodd}{isodd(\j) && \j > 1 && \j <= \n}
                \pgfmathsetmacro{\xeven}{iseven(\j) && \j > 1 && \j <= \n}
                \ifthenelse{\xodd=1}{
                    \node[rotate=8,regular polygon,regular polygon sides=#1,minimum
                    size=\j*35pt] (p\j) {};
                    }{
                    \ifthenelse{\xeven=1}{
                        \draw[\es,double=black!20] circle (\j*17.6pt);
                        \node[rotate=-10/\j,regular polygon,regular polygon sides=#1,minimum
                        size=\j*35pt] (p\j) {};
                        }{
                        \node[regular polygon,regular polygon sides=#1,minimum
                        size=\j*35pt] (p\j) {};
                    }
                }

                \foreach\l in {1,...,#1}{
                    \pgfmathsetmacro{\de}{(9 * \l + 7.4) * 40 / #1}
                    \pgfmathsetmacro{\dee}{(9 * \l + 6) * 40 / #1}
                    \draw[very thick,white] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                    \draw[thick,dotted,black!20] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                    \node[inner sep=1.8pt, circle,fill= white] (\j\l) at (p\j.corner \l) {};
                    \ifthenelse{\xeven=1}{
                        \node[\vs,black!20] (\j\l) at (p\j.corner \l) {};
                    }{}
                }
            }
            \foreach\j in {1,...,#1} {
                \foreach\l in {1,...,#1}{

                \pgfmathsetmacro{\xeven}{iseven(\j) && \j > 2}
                \pgfmathsetmacro{\xodd}{isodd(\j) && \j > 2}
                \pgfmathsetmacro{\jmt}{int(\j - 2)}
                \ifthenelse{\xeven=1}{
                    \dotedge[\es,double=black!20](\j\l)--(\jmt\l);
                }{}
                \ifthenelse{\xodd=1}{
                    \dotedge[\es,double=black](\j\l)--(\jmt\l);
                }{}
            }
            \dotedge[\es,double=black!20](#1\j)--(\n\j);
            \dotedge[\es,double=black!20](1\j)--(2\j);
        }
        \foreach\j in {1,...,#1} {
                \pgfmathsetmacro{\xeven}{iseven(\j) && \j > 1 && \j <= \n}
                \ifthenelse{\xeven=1}{}{
                    \draw[\es] circle (\j*17.6pt);
                    \foreach\l in {1,...,#1}{
                        \node[inner sep=1.8pt, circle,fill= white] (\j\l) at (p\j.corner \l) {};
                        \node[\vs] (\j\l) at (p\j.corner \l) {};
                        \ifthenelse{\j=1}{
                            \pgfmathsetmacro{\de}{(9 * \l + 9) * 40 / #1}
                            \pgfmathsetmacro{\dee}{(9 * \l + 4.5) * 40 / #1}
                            }{
                            \pgfmathsetmacro{\de}{(9 * \l + 7.5) * 40 / #1}
                            \pgfmathsetmacro{\dee}{(9 * \l + 6.1) * 40 / #1}
                        }
                        \draw[very thick,white] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                        \draw[thick,dotted] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                    }
                }
            }
        }
    }
}
\tikzset{
    pics/grid/.style args={#1/#2}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\sty,10))}
            \pgfmathsetmacro{\mode}{int(\sty - \bg * 10)}

            \pgfmathsetmacro{\normalgrid}{#2==14}
            \ifthenelse{\mode=0}{
                % normal mode
                \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                \ifthenelse{\normalgrid=1}{
                    \def\vs{tvertex}
                    }{
                    \def\vs{btvertex}
                }
                \def\es{tedge}
                \def\ess{stedge}
                }{
                \ifthenelse{\mode=1}{
                    % grid where each vertex is split into 6 parts (for a 3d grid
                    \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                    \ifthenelse{\normalgrid=1}{
                        \def\vs{tvertex}
                        }{
                        \def\vs{bbtvertex}
                    }
                    \def\es{tedge}
                    \def\ess{stedge}
                    }{
                    % grid-colored graph (only supports 2d grids
                    \pgfmathsetmacro{\dist}{\bg==2?1.15:.9}
                    \def\vs{bag}
                    \def\es{dedge}
                    \def\ess{sdedge}
                }
            }
            \pgfmathsetmacro{\n}{int(#1-1)}
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\xedgee}{\i==\n}
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \node[\vs] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\xedgee=1}{
                        \draw[smooth,\ess]
                        (\j\l.east)
                        to ($(\j\l.east) + (.35, 0)$)
                        to[out=0, in=0] ($(\j\l.east) + (.35, -0.25)$)
                        to ($(1\l.west) - (.15, 0.25)$)
                        to[out=180,in=180] ($(1\l.west) - (.15, 0)$)
                        to (1\l.west)
                        ;
                    }{}
                    }{
                    \node[inner sep=1.3ex] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\yodd=1}{
                        \draw[dotted,\es] (\j\l.west) -- (\j\l.east);
                        }{
                        \ifthenelse{\xodd=1}{
                            \draw[dotted,\es] (\j\l.north) -- (\j\l.south);
                            }{
                }}}
            }
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \node[\vs] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\yedgee=1}{
                        \draw[smooth,\ess]
                        (\j\l.north)
                        to ($(\j\l.north) + (0,.15)$)
                        to[out=90, in=90] ($(\j\l.north) + (.25, 0.15)$)
                        to ($(\j1.south) - (-.25, 0.35)$)
                        to[out=270,in=270] ($(\j1.south) - (0,.35)$)
                        to (\j1.south)
                        ;
                    }{}
                    }{
                    \node[inner sep=1.3ex] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\yodd=1}{
                        \draw[dotted,\es] (\j\l.west) -- (\j\l.east);
                        }{
                        \ifthenelse{\xodd=1}{
                            \draw[dotted,\es] (\j\l.north) -- (\j\l.south);
                            }{
                }}}
            }
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\xedge}{\i==-\n || \i==\n}
                \pgfmathsetmacro{\yedge}{\k==-\n || \k==\n}
                \pgfmathsetmacro{\xedgee}{\i==\n}
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\corner}{\xedge && \yedge}
                \pgfmathsetmacro{\edge}{\xedge || \yedge}

                \ifthenelse{\corner=1}{\def\tp{corner}}
                {\ifthenelse{\edge=1}{\def\tp{edge}}
                {\def\tp{inner}}}

                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \ifthenelse{\normalgrid=1}{
                        \node[\vs] (\j\l) at (\dist*\i,\dist*\k) {};
                        }{
                        \ifthenelse{\mode=0}{
                            \node[ssvertex] (n\j\l) at ($(\j\l.north)+(0,-.065)$) {};
                            \node[ssvertex] (e\j\l) at ($(\j\l.east)+(-.065,0)$) {};
                            \node[ssvertex] (s\j\l) at ($(\j\l.south)+(0,.065)$) {};
                            \node[ssvertex] (w\j\l) at ($(\j\l.west)+(.065,0)$) {};

                            % \draw[ssedge] (n\j\l) -- (s\j\l);
                            % \draw[ssedge] (s\j\l) -- (e\j\l);
                            }{
                            \node[sssvertex] (ne\j\l) at ($(\j\l.north east)+(-0.05,-.05)$) {};
                            \node[ssvertex] (n\j\l) at ($(\j\l.north)+(0,-.06)$) {};
                            \node[ssvertex] (e\j\l) at ($(\j\l.east)+(-.06,0)$) {};
                            \node[ssvertex] (s\j\l) at ($(\j\l.south)+(0,.06)$) {};
                            \node[ssvertex] (w\j\l) at ($(\j\l.west)+(.06,0)$) {};
                            \node[bbvertex] (sw\j\l) at ($(\j\l.south west)-(-0.05,-.05)$) {};

                            \ifthenelse{#2=15}{
                                \draw[tedge] (ne\j\l) -- (sw\j\l);
                                \draw[sssedge] (w\j\l) -- (n\j\l) -- (e\j\l) -- (s\j\l);
                            }{}
                            \ifthenelse{#2=16}{
                                \draw[tedge] (w\j\l) -- (ne\j\l);
                                \draw[sssedge] (n\j\l) -- (s\j\l);
                                \draw[tedge] (ne\j\l) -- (e\j\l) -- (sw\j\l) -- (w\j\l);
                                \node[ssvertex] (n\j\l) at ($(\j\l.north)+(0,-.06)$) {};
                            }{}
                            \ifthenelse{#2=17}{
                                \draw[tedge] (s\j\l) -- (ne\j\l);
                                \draw[sssedge] (w\j\l) -- (e\j\l);
                                \draw[tedge] (sw\j\l) -- (n\j\l) -- (ne\j\l)  (s\j\l) -- (sw\j\l);
                                \node[ssvertex] (e\j\l) at ($(\j\l.east)+(-.06,0)$) {};
                            }{}
                        }
                        \ifthenelse{#2=1}{\draw[ssedge] (n\j\l) -- (s\j\l);}{}
                        \ifthenelse{#2=2}{\draw[ssedge] (w\j\l) -- (e\j\l);}{}
                        \ifthenelse{#2=3}{\draw[ssedge] (n\j\l) -- (e\j\l);}{}
                        \ifthenelse{#2=4}{\draw[ssedge] (s\j\l) -- (e\j\l);}{}
                        \ifthenelse{#2=5}{\draw[ssedge] (n\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=6}{\draw[ssedge] (s\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=7}{\draw[ssedge] (n\j\l) -- (e\j\l);
                        \draw[ssedge] (s\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=8}{\draw[ssedge] (s\j\l) -- (e\j\l);
                        \draw[ssedge] (n\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=9}{
                            \draw[ssedge] (e\j\l) -- (w\j\l);
                            \draw[ssedge] (s\j\l) -- (n\j\l);
                        }{}
                        \ifthenelse{#2=10}{\draw[ssedge] (n\j\l) -- (e\j\l) -- (s\j\l);}{}
                        \ifthenelse{#2=11}{\draw[ssedge] (e\j\l) -- (s\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=12}{\draw[ssedge] (s\j\l) -- (w\j\l) -- (n\j\l);}{}
                        \ifthenelse{#2=13}{\draw[ssedge] (w\j\l) -- (n\j\l) -- (e\j\l);}{}

                    }
                    \ifthenelse{\j>1}{
                        \pgfmathsetmacro{\up}{int(\j-1)}
                        \pgfmathsetmacro{\upp}{int(\j-2)}
                        \draw[\es] (\up\l) -- (\j\l);
                        \draw[\es] (\upp\l) -- (\up\l);
                    }{}
                    \ifthenelse{\l>1}{
                        \pgfmathsetmacro{\left}{int(\l-1)}
                        \pgfmathsetmacro{\leftt}{int(\l-2)}
                        \draw[\es] (\j\left) -- (\j\l);
                        \draw[\es] (\j\left) -- (\j\leftt);
                    }{}

                }{}
            }
        }
    }
}

\tikzset{
    pics/gridgrid/.style args={#1/#2}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\sty,10))}
            \pgfmathsetmacro{\mode}{int(\sty - \bg * 10)}
            \begin{scope}[opacity=0.4]
                \begin{scope}[opacity=0.2]
                    \pic[sty=\bg1] (2) at (2, 2) {grid=#1/#2};
                \end{scope}
                \pic[sty=\bg1] (1) at (1, 1) {grid=#1/#2};
            \end{scope}
            \pic[sty=\bg1] (0) at (0, 0) {grid=#1/#2};

            \pgfmathsetmacro{\normalgrid}{#2==14}
            \pgfmathsetmacro{\n}{int(#1-1)}
            \ifthenelse{\mode=0}{
                % normal mode
                \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                \ifthenelse{\normalgrid=1}{
                    \def\vs{tvertex}
                    }{
                    \def\vs{btvertex}
                }
                \def\es{tedge}
                \def\ess{stedge}
                }{
                \ifthenelse{\mode=1}{
                    % grid where each vertex is split into 6 parts (for a 3d grid
                    \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                    \ifthenelse{\normalgrid=1}{
                        \def\vs{tvertex}
                        }{
                        \def\vs{bbtvertex}
                    }
                    \def\es{tedge}
                    \def\ess{stedge}
                    }{
                    % grid-colored graph (only supports 2d grids
                    \pgfmathsetmacro{\dist}{\bg==2?1.15:.9}
                    \def\vs{bag}
                    \def\es{dedge}
                    \def\ess{sdedge}
                }
            }

            \definecolor{l2b}{rgb}{.6,.6,.6}
            \definecolor{l1b}{rgb}{.8,.8,.8}
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\xedge}{\i==-\n || \i==\n}
                \pgfmathsetmacro{\yedge}{\k==-\n || \k==\n}
                \pgfmathsetmacro{\xedgee}{\i==\n}
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\corner}{\xedge && \yedge}
                \pgfmathsetmacro{\edge}{\xedge || \yedge}

                \ifthenelse{\corner=1}{\def\tp{corner}}
                {\ifthenelse{\edge=1}{\def\tp{edge}}
                {\def\tp{inner}}}

                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \ifthenelse{\normalgrid=1}
                    {

                        \draw[\es,double=black!60,dotted]  ($(0\j\l)!0.35!(1\j\l)$) --
                        ($(0\j\l)!0.64!(1\j\l)$);
                        \draw[\es,double=black!30,dotted]  ($(1\j\l)!0.35!(2\j\l)$) --
                        ($(1\j\l)!0.64!(2\j\l)$);
                        \draw[\es,double=black] (0\j\l) -- ($(0\j\l)!0.37!(1\j\l)$);
                        \draw[\es,double=black!40] (1\j\l) -- ($(0\j\l)!0.62!(1\j\l)$);

                        \draw[\es,double=black!40] (1\j\l) -- ($(1\j\l)!0.37!(2\j\l)$);
                        \draw[\es,double=black!20] (2\j\l) -- ($(1\j\l)!0.62!(2\j\l)$);
                        \draw[smooth,\ess]
                        (2\j\l.north east)
                        to ($(2\j\l.north east) + (.15,.15)$)
                        to[out=45, in=45] ($(2\j\l.north east) + (.45, 0.15)$)
                        to ($(0\j\l.south west) - (-0.05, 0.25)$)
                        to[out=270-45,in=270-45] ($(0\j\l.south west) - (.25,.25)$)
                        to (0\j\l.south west)
                        ;
                        }{
                        \draw[\es,double=black!60,dotted]  ($(0\j\l)!0.35!(1\j\l)$) --
                        ($(0\j\l)!0.64!(1\j\l)$);
                        \draw[\es,double=black!30,dotted]  ($(1\j\l)!0.35!(2\j\l)$) --
                        ($(1\j\l)!0.64!(2\j\l)$);
                        \draw[\es,double=black] (0\j\l) -- ($(0\j\l)!0.37!(1\j\l)$);
                        \draw[\es,double=black!40] (1\j\l) -- ($(0\j\l)!0.62!(1\j\l)$);

                        \draw[\es,double=black!40] (1\j\l) -- ($(1\j\l)!0.37!(2\j\l)$);
                        \draw[\es,double=black!20] (2\j\l) -- ($(1\j\l)!0.62!(2\j\l)$);
                        \draw[smooth,sstedge]
                        ($(2\j\l.north east) - (.02,.02)$)
                        to ($(2\j\l.north east) + (.05,.05)$)
                        to[out=45, in=45] ($(2\j\l.north east) + (.35, 0.05)$)
                        to ($(0\j\l.south west) - (-0.15, 0.15)$)
                        to[out=270-45,in=270-45] ($(0\j\l.south west) - (.15,.15)$)
                        to (0\j\l.south west)
                        ;

                    }
                }{}
            }

        }
    }
}


\makeatother

